Pricing Security in Proof-of-Work Systems

A key component of security in decentralized blockchains is proof of opportunity cost among block producers. In the case of proof-of-work (PoW), currently used by the most prominent systems, the cost is due to spent computation. In this paper, we characterize the security investment of miners in terms of its cost in fiat money. This enables comparison of security allocations across PoW blockchains that generally use different PoW algorithms and reward miners in different cryptocurrency units. We prove that there exists a unique allocation equilibrium, depending on market prices only, that is achieved by both strategic miners (who contemplate the actions of others) and by miners seeking only short-term profit. In fact, the latter will unknowingly compensate for any attempt to deliberately shift security allocation away from equilibrium. Our conclusions are supported analytically through the development of a Markov decision process, game theoretical analysis, and derivation of no arbitrage conditions. We corroborate those results with empirical evidence from more than two years of blockchain and price data. Overall agreement is strong. We show that between January 1, 2018 and August 1, 2020, market prices predicted security allocation between Bitcoin and Bitcoin Cash with error less than 0.6%. And from the beginning of October 2019, until August 1, 2020, market prices predicted security allocation between Bitcoin and Litecoin with error of 0.45%. These results are further corroborated by our establishment of Granger-causality between change in market prices and change in security allocation. To demonstrate the practicality of our results, we describe a trustless oracle that leverages the equilibrium to estimate the price ratios of PoW cryptocurrencies from on-chain information only.

==> ack.tex <==
% !TEX root = main.tex

\section{Acknowledgements}

We would like to thank David Jensen and Akanksha Atrey for many thought provoking discussions, which helped us to focus our investigation. We would also like to thank Rainer B{\"o}hme for his insights in the discussions we had with him.

==> econometrics/applications.tex <==
% !TEX root = main.tex

\section{Applications}

\begin{figure}[t]
   \centering
   \includegraphics[width=0.8\columnwidth]{figures/futures} 
   \caption{Performance of Futures based on PoW-based price estimation.}
   \label{fig:example}
\end{figure}
\subsection{Supporting Atomic Swaps, Lightning Networks, and Futures without Inequities}

Atomic swaps~\cite{Atmoic_swap} allow two opposing parties to exchange two distinct coins: Alice gives quantity $c_A$ of the coin native to blockchain $A$ to Bob, who in exchange gives quantity $c_B$ of the coin native to blockchain $B$. Such protocols are designed to achieve a {\em fair exchange}~\cite{Asokan:1997} between two parties: either the exchange executes or not, that is, neither party can lose coins as a result of a failed execution. 

Unfortunately, one party can abuse the process to turn it into an inadvertent options mechanism~\cite{Bitmex:2019}. Lightning networks that allow exchange of coin between two currencies have the same problem~\cite{Plooy:2018}. Existing solutions make use of a trusted third party.  For the same reasons, futures contracts are also problematic. Below, we explain the problem and our solution, which does not use a third party.

An atomic swap works as follows. Alice and Bob setup the safeguards for the swap. A hash time locked contract (HTLC) contract is used that allows for Alice and Bob to each place funds in a multi-sig address without waiting for the other party to initiate.  If one party doesn't complete the exchange, then at the end of the lock deadline, the other  party is returned their funds from the multi-sig address. However, the value of coin $A$, $P_A$, may fall relative to that of coin $B$, $P_B$. In this case, Alice can make a decision to back out. Thus, she can leverage Bob's holdings as an {\em option} that she unilaterally controls~\cite{Plooy:2018,Bitmex:2019}. In other words, there are three cases: \1 Alice can back out, abusing the purpose of the HTLC to protect her funds against a fall in value; \2 she can proceed with the swap, but she will receive less than the exchange rate of $P_A / P_B$ that was encoded;  \3 she can proceed, but due to a change of the exchange rate, Bob  receives less than $c_A$ coins for his $c_B$. 

Thus, Atomic swaps are only a fair exchange if either: the value of the two coins does not change, which is a condition that cannot be guaranteed; or the value of the exchange changes with the market. Changes in exchange rates can be mitigated by reducing the length of the deadline. But cryptocurrency markets have a history of variability. Furthermore, it is because of this problem that {\em futures contracts} cannot be supported in cryptocurrencies: the typical lengths of futures (day and months) exacerbate this problem. 


%To remove the inequity, the amount of coin Alice finally receives from Bob should be based on the exchange rate at the time that Alice proceeds with the final step of the swap and not the rate when the swap initiated. 

Our solution is to construct a contract that accepts block headers of both coins, which can be validated as real POW in a contract. The ratio of the hash rates is a linear factor in the final exchange rates. 

\reminder{sketch:}

- Alice and Bob agree upon the latest block header from coin A and coin B. They agree upon all parameters used below. cA, cB, m, and z. length of contract.

- Alice places cA*m in contract, bob places cB*m. The margin is m

- At the end of the contract,  either party can submit all headers from both coins to the contract, plus $z$ more (to prevent a doublespend-like attack). It validates all headers (sans transactions, like a lite client). 

- The contract uses Theorem 1 to estimate the exchange rate, and adjusts the payout accordingly

- if at any time, the payout is greater than cA*m or cB*m, there is a margin call and the contract closes.

- An attack based on falsified difficulty and timestamps can allow one party to falsify things. We need to explain the details of how to avoid that. One answer is to make use of the expected block times and therefore height and use the height of the contract itself to monitor it. need to write this out in detail.







\reminder{random idea: A coin could be programmed to offer futures on its coinbase. Or even take x\% of its future coinbase and sell it as a futures contract for another coin.}


%TODO: adjust lightning protocol
%
%\url{https://lists.linuxfoundation.org/pipermail/lightning-dev/2018-December/thread.html#1752}
%
%\url{https://lists.linuxfoundation.org/pipermail/lightning-dev/2018-December/001752.html}
%\url{https://lists.linuxfoundation.org/pipermail/lightning-dev/2018-May/001292.html}
%
%\url{https://bitonic.nl/public/slowdown_prevention.pdf}
%
% This is about looping, not the same problem: \url{https://bitcointechweekly.com/front/preventing-delay-abuse-in-a-lightning-based-peer-to-peer-exchange/}




==> econometrics/fig/gof-2018-eth-etc.tex <==
$ 0.0059$&$ 0.0042$&$-0.0041$&$44.6357$

==> econometrics/fig/gof-2018-h192.tex <==
$ 0.0111$&$ 0.0070$&$ 0.0013$&$39.0595$

==> econometrics/fig/gof-2018-h96.tex <==
$ 0.0126$&$ 0.0081$&$ 0.0028$&$38.0153$

==> econometrics/fig/gof-2018-target.tex <==
$ 0.0102$&$ 0.0062$&$ 0.0003$&$39.8533$

==> econometrics/fig/gof-2019-eth-etc.tex <==
$ 0.0042$&$ 0.0021$&$ 0.0011$&$47.4325$

==> econometrics/fig/gof-2019-h192.tex <==
$ 0.0020$&$ 0.0014$&$ 0.0001$&$54.1788$

==> econometrics/fig/gof-2019-h96.tex <==
$ 0.0021$&$ 0.0016$&$ 0.0005$&$53.4714$

==> econometrics/fig/gof-2019-target.tex <==
$ 0.0018$&$ 0.0013$&$-0.0002$&$54.8992$

==> econometrics/fig/gof-2020-eth-etc.tex <==
$ 0.0033$&$ 0.0024$&$-0.0012$&$49.5641$

==> econometrics/fig/gof-2020-h192.tex <==
$ 0.0020$&$ 0.0015$&$ 0.0000$&$53.7955$

==> econometrics/fig/gof-2020-h96.tex <==
$ 0.0023$&$ 0.0017$&$ 0.0001$&$52.6818$

==> econometrics/fig/gof-2020-target.tex <==
$ 0.0018$&$ 0.0012$&$ 0.0000$&$54.9855$
